Nonequilibrium quantum states emerging from flippable spins in random networks

Recent advances in programmable quantum simulators have enabled the realization of irregular interaction networks, which natural crystal lattices cannot provide, together with time-resolved observation of quantum many-body dynamics. Understanding the nonequilibrium states that emerge from such networks has only just begun, and whether quantum many-body scar states can emerge in them remains open. Here, focusing on a quantum Ising spin system with random interaction networks under a weak transverse field, we introduce the flippability, the fraction of flippable spins, and present phenomenological laws that predict the emergence of quantum many-body scar states from the network structure. As the flippability increases, the Hilbert space becomes less fragmented. The largest kinetically accessible subspace shows nonintegrable level statistics, yet hosts a few eigenstates with abnormally low participation entropy, signalling scar states. Real-time dynamics from Fock states confirm these signatures: systems with higher flippability tend toward thermalization, whereas a few initial states show anomalously nonthermal dynamics. The flippability thus links the interaction-network structure of the Hamiltonian to nonequilibrium many-body dynamics without translational invariance, and may apply to other kinetically constrained quantum systems.

==> preamble-commons.tex <==
\usepackage{cmap}
\usepackage[T1]{fontenc}
\usepackage{newtxtext}% Times New Roman font
\usepackage[varvw]{newtxmath}% Times New Roman font for math
\usepackage{microtype}
\usepackage{graphicx}% Include figure files
\graphicspath{{figures/}}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{hyperref}% add hypertext capabilities
\hypersetup{colorlinks=true,allcolors=blue}
\urlstyle{same}
%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines
\usepackage{mathtools}% for \coloneqq
\usepackage{upgreek}% for upright pi
\usepackage{cancel}
\usepackage{braket}
\usepackage{makecell}
\usepackage{orcidlink}
\allowdisplaybreaks

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argwhere}{arg\,where}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\med}{med}
